A Formal Framework of Virtual Organisations as Agent Societies

We propose a formal framework that supports a model of agent-based Virtual Organisations (VOs) for service grids and provides an associated operational model for the creation of VOs. The framework is intended to be used for describing different service grid applications based on multiple agents and, as a result, it abstracts away from any realisation choices of the service grid application, the agents involved to support the applications and their interactions. Within the proposed framework VOs are seen as emerging from societies of agents, where agents are abstractly characterised by goals and roles they can play within VOs. In turn, VOs are abstractly characterised by the agents participating in them with specific roles, as well as the workflow of services and corresponding contracts suitable for achieving the goals of the participating agents. We illustrate the proposed framework with an earth observation scenario.

==> eptcsdata.tex <==
\providecommand{\event}{Jeremy W. Bryans and John S. Fitzgerald (Eds.): \\
Formal Aspects of Virtual Organisations 2009 (FAVO2009)}
\providecommand{\volume}{16}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{1}
\providecommand{\eid}{1}
\pdfoutput=1

